2024 NSF CSSI-Cybertraining-SCIPE PI Meeting August 12 to 13, 2024, Charlotte, NC

The second annual NSF, OAC CSSI, CyberTraining and related programs PI meeting was held August 12 to 13 in Charlotte, NC, with participation from PIs or representatives of all major awards. Keynotes, panels, breakouts, and poster sessions allowed PIs to engage with each other, NSF staff, and invited experts. The 286 attendees represented 292 awards across CSSI, CyberTraining, OAC Core, CIP, SCIPE CDSE, and related programs, and presented over 250 posters. This report documents the meetings structure, findings, and recommendations, offering a snapshot of current community perspectives on cyberinfrastructure. A key takeaway is a vibrant, engaged community advancing science through CI. AI-driven research modalities complement established HPC and data centric tools. Workforce development efforts align well with the CSSI community.

==> breakout/II_01_open_science.tex <==
%%% section: II_01_Open Science and CSSI
\label{sec:breakout2_1}

Leads:  \\
Main Facilitator:  Name, Org \\
Scribes:   Name, Org \\
  Name, Org  \\


Notes can be found here: \href{https://docs.google.com/document/d/1cAzFVpJQ6_L_EpJyAKREM7dUteg-zYzr7vPeSi1z9pI/edit?tab=t.0}{[meeting notes]}


Link to Breakout report: 
\href{https://docs.google.com/document/d/1FB5drrM986Pj3HKk5OCTMQahhPGyTcApr-AxubUobV0/edit?tab=t.0#heading=h.8tpgz3aom6fa}
{[Open Science and CSS -  Guoyu]}

\subsubsection{Summary}

\subsubsection{Desired Outcomes / Future Directions}
\label{sec:breakout2_1-fut}
TBD

\subsubsection{Recommendations}
\label{sec:breakout2_1-rec}
TBD
